Template-Driven LLM-Paraphrased Framework for Tabular Math Word Problem Generation

Solving tabular math word problems (TMWPs) has become a critical role in evaluating the mathematical reasoning ability of large language models (LLMs), where large-scale TMWP samples are commonly required for LLM fine-tuning. Since the collection of high-quality TMWP datasets is costly and time-consuming, recent research has concentrated on automatic TMWP generation. However, current generated samples usually suffer from issues of either correctness or diversity. In this paper, we propose a Template-driven LLM-paraphrased (TeLL) framework for generating high-quality TMWP samples with diverse backgrounds and accurate tables, questions, answers, and solutions. To this end, we first extract templates from existing real samples to generate initial problems, ensuring correctness. Then, we adopt an LLM to extend templates and paraphrase problems, obtaining diverse TMWP samples. Furthermore, we find the reasoning annotation is important for solving TMWPs. Therefore, we propose to enrich each solution with illustrative reasoning steps. Through the proposed framework, we construct a high-quality dataset TabMWP-TeLL by adhering to the question types in the TabMWP dataset, and we conduct extensive experiments on a variety of LLMs to demonstrate the effectiveness of TabMWP-TeLL in improving TMWP solving performance. The code and data of this paper are available at: https://github.com/Jason8Kang/TELL.

==> Figures/Generalization.tex <==
\begin{figure}[t!]
    \begin{tcolorbox}[
    %title=Prompt for Template Generalization, 
    left=2mm,right=1mm,top=0mm, bottom=0mm,colback=white,colframe=NavyBlue]
    \begin{lstlisting}[style=plain]
You are given a question and answer with tabular contents, and your task is to develop a versatile exercise template that can generate a wide array of exercises with a table. Please consider the following guidelines for this assignment:

(1) You can use pandas, numpy, random, etc. or other packages if necessary.
(2) You should construct a general dataframe and transform it into a human-readable table format by Python.
(3) Generate the functions that are used to create the question, answer, and step-by-step solution based on the created table.

This is an demonstration for <Task 1>:
<Demonstration for Task 1>
Please generate the exercise template for <Task 2>.
    \end{lstlisting}
    \end{tcolorbox}
    \caption{Prompt for template augmentation.}
    \label{fig:generalization}
\end{figure}

==> Figures/Paraphrase.tex <==
\begin{figure}[t!]
    \begin{tcolorbox}[
    %title=Prompt for Natural Question Paraphrasing, 
    left=2mm,right=1mm,top=0mm, bottom=0mm,colback=white,colframe=OliveGreen]
    \begin{lstlisting}[style=plain]
You need to rewrite the given math word problem to increase data diversity and semantic richness, whose questions and solutions are generated according to a uniform template. You should keep the original problem, data, and solution logic unchanged. Specific requirements are as follows:

(1) Question (`question`): You need to add a background to the question, set the problem in a specific scenario before introducing the question, and rewrite the question without changing its original meaning.

(2) Solution (`solution`): Since a background has been introduced to the question, the solution process should also be correspondingly rewritten, but the idea and logic should remain the same. You can appropriately modify any unreasonable parts in the reasoning process based on the actual situation.

(3) Table Content (`table_for_pd`), Choices (`choices`), and Answer (`answer`): These parts should remain unchanged unless the keys of the tables and the choices and answers for multiple-choice questions.

Here are two examples:
<Two In-context Examples>

Please rewrite the following question based on the aforementioned requirements and examples:
<Template-based Question>
    \end{lstlisting}
    \end{tcolorbox}
    \caption{Prompt for paraphrasing template-based problems to natural problems.}
    \label{fig:paraphrase}
\end{figure}

==> Tables/Ablation.tex <==
\begin{table}[t!]
    \centering
    \small
    \begin{tabular}{l|cccc}
        \toprule
        \textbf{Model} & \textbf{FREE} & \textbf{MC} & \textbf{Overall} & $\mathbf{\Delta}$ \\
        \midrule
        Mistral & $90.87$ & $97.79$ & $92.66$ & $-$ \\
        \quad \textit{w/ Template} & $91.41$ & $98.29$ & $93.20$ & $0.54$ \\
        \quad \textit{w/ Ques.+Table} & $91.27$ & $97.64$ & $92.92$ & $0.26$ \\
        \quad \textit{w/ Ques. Only} & $92.48$ & $\mathbf{98.64}$ & $94.08$ & $1.42$ \\
        \quad \textit{Ours} & $\mathbf{96.08}$ & $98.14$ & $\mathbf{96.62}$ & $\mathbf{3.96}$ \\        
        \midrule
        Qwen 2 & $92.10$ & $97.84$ & $93.59$ & $-$ \\
        \quad \textit{w/ Template} & $92.20$ & $\mathbf{98.19}$ & $93.75$ & $0.16$ \\
        \quad \textit{w/ Ques.+Table} & $92.48$ & $97.79$ & $93.86$ & $0.27$ \\
        \quad \textit{w/ Ques. Only} & $93.47$ & $97.84$ & $94.60$ & $1.01$ \\
        \quad \textit{Ours} & $\mathbf{97.07}$ & $97.94$ & $\mathbf{97.29}$ & $\mathbf{3.70}$ \\
        \midrule
        Llama 3 & $94.13$ & $94.73$ & $94.29$ & $-$ \\
        \quad \textit{w/ Template} & $93.08$ & $97.99$ & $94.35$ & $0.06$ \\
        \quad \textit{w/ Ques.+Table} & $93.26$ & $98.24$ & $94.55$ & $0.26$ \\
        \quad \textit{w/ Ques. Only} & $94.33$ & $98.69$ & $95.46$ & $1.17$ \\
        \quad \textit{Ours} & $\mathbf{97.91}$ & $\mathbf{98.54}$ & $\mathbf{98.07}$ & $\mathbf{3.78}$ \\
        \bottomrule
    \end{tabular}
    \caption{Comparison of different TMWP generation methods. $\mathbf{\Delta}$ calculates the overall improvement.}
    \label{tab:ablation}
\end{table}

==> Tables/Results.tex <==
% --------------------
% Notations:
% TP: Template-based Question (题目模板)
% QP: Question Paraphrase (问题/表格数字改写)
% LP: LLM Question Paraphrase (大模型同义问题改写)
% --------------------
\begin{table*}[t!]
    \centering
    \small
    \begin{tabular}{l|cccccccccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\#Para.}} & \multicolumn{2}{c}{\textbf{Question Type}} & & \multicolumn{5}{c}{\textbf{Answer Type}} & & \multicolumn{2}{c}{\textbf{Grade}} & & \multirow{2}{*}{\textbf{Avg.}} \\
        \cmidrule{3-4} \cmidrule{6-10} \cmidrule{12-13}
         & & FREE & MC & & INT & DEC & EXTR & BOOL & OTH & & 1-6 & 7-8 & \\
        \midrule
        \rowcolor{gray!10} & \multicolumn{14}{c}{\textit{Heuristic Baselines}} \\
        \midrule
        Heuristic Guess & $-$ & $6.71$ & $39.81$ & & $8.37$ & $0.26$ & $30.80$ & $51.22$ & $26.67$ & & $17.55$ & $12.27$ & & $15.29$ \\
        Human Perform. & $-$ & $84.61$ & $93.32$ & & $84.95$ & $83.29$ & $97.18$ & $88.69$ & $96.20$ & & $94.27$ & $81.28$ & & $90.22$ \\
        \midrule
        \rowcolor{gray!10} & \multicolumn{14}{c}{\textit{Fine-tuned LMs}} \\
        \midrule
        UnifiedQA$_\textsc{large}$ & $770$M & $48.67$ & $82.18$ & & $55.97$ & $20.26$ & $94.63$ & $68.89$ & $79.05$ & & $65.92$ & $45.92$ & & $57.35$ \\
        TAPEX$_\textsc{large}$ & $400$M & $51.00$ & $80.02$ & & $59.92$ & $16.31$ & $95.34$ & $64.00$ & $73.33$ & & $67.11$ & $47.07$ & & $58.52$ \\
        TaCo$_\textsc{large}$ & $800$M & $91.69$ & $93.47$ & & $92.54$ & $88.41$ & $96.05$ & $91.44$ & $86.67$ & & $92.37$ & $91.86$ & & $92.15$ \\ 
        \midrule
        \rowcolor{gray!10} & \multicolumn{14}{c}{\textit{Few-shot Prompting}} \\
        \midrule
        GPT-3 & $175$B & $54.69$ & $64.11$ & & $58.36$ & $40.40$ & $75.95$ & $52.41$ & $53.02$ & & $63.10$ & $49.16$ & & $57.13$ \\
        ChatGPT & $20$B & $65.84$ & $64.61$ & & $66.55$ & $63.09$ & $74.67$ & $54.67$ & $55.24$ & & $69.75$ & $59.88$ & & $65.52$ \\
        \midrule
        \rowcolor{gray!10} & \multicolumn{14}{c}{\textit{Few-shot CoT Prompting}} \\
        \midrule
        Mistral & $7$B & $47.32$ & $48.34$ & & $47.62$ & $46.17$ & $48.30$ & $48.87$ & $44.09$ & & $47.66$ & $47.49$ & & $47.59$ \\
        Qwen 2 & $7$B &  $67.84$ & $68.44$ & & $68.06$ & $66.94$ & $68.12$ & $69.49$ & $62.56$ & & $67.94$ & $68.06$ & & $67.99$ \\
        Llama 3 & $8$B & $71.87$ & $72.34$ & & $72.35$ & $70.00$ & $72.36$ & $72.91$ & $67.12$ & & $72.36$ & $71.51$ & & $71.99$ \\
        GPT-3 & $175$B & $60.76$ & $69.09$ & & $60.04$ & $63.58$ & $76.49$ & $69.19$ & $67.30$ & & $68.62$ & $55.31$ & & $62.92$ \\
        ChatGPT & $20$B & $80.89$ & $87.50$ & & $79.36$ & $86.87$ & $81.86$ & $94.00$ & $84.76$ & & $82.68$ & $82.51$ & & $82.60$ \\
        GPT-4 & $1.8$T$^*$ & $90.81$ & $88.48$ & & $97.49$ & $86.16$ & $97.51$ & $96.86$ & $99.11$ & & $89.52$ & $92.40$ & & $88.70$ \\
        PromptPG & $175$B & $66.17$ & $74.11$ & & $64.12$ & $74.16$ & $76.19$ & $72.81$ & $65.81$ & & $71.20$ & $64.27$ & & $68.23$ \\
        PoT (GPT-4) & $1.8$T$^*$ & $97.40$ & $95.58$ & & $98.48$ & $93.22$ & $96.25$ & $98.00$ & $68.57$ & & $96.97$ & $96.87$ & & $96.93$ \\
        Chameleon & $1.8$T$^*$ & $98.95$ & $98.29$ & & $99.34$ & $97.42$ & $98.58$ & $98.56$ & $93.33$ & & $98.95$ & $98.54$ & & $98.78$ \\
        \midrule
        \rowcolor{gray!10} & \multicolumn{14}{c}{\textit{Fine-tuned LLMs}} \\
        \midrule
        Mistral & $7$B & $90.87$ & $97.79$ & & $90.93$ & $90.64$ & $97.77$ & $99.44$ & $83.81$ & & $92.67$ & $92.65$ & & $92.66$ \\
        Qwen 2 & $7$B & $92.10$ & $97.84$ & & $92.54$ & $90.39$ & $96.76$ & $99.67$ & $92.38$ & & $94.24$ & $92.71$ & & $93.59$ \\
        Llama 3 & $8$B & $94.13$ & $94.73$ & & $94.81$ & $91.50$ & $98.78$ & $90.11$ & $96.19$ & & $96.61$ & $91.19$ & & $94.29$ \\
        \midrule
        \rowcolor{gray!10} & \multicolumn{14}{c}{\textit{Ours (Trained with TabMWP + TabMWP-TeLL)}} \\
        \midrule
        Mistral & $7$B & $96.08$ & $98.14$ & & $96.69$ & $93.73$ & $98.07$ & $99.22$ & $89.52$ & & $96.77$ & $96.42$ & & $96.62$ \\
        Qwen 2 & $7$B & $97.07$ & $97.94$ & & $97.39$ & $\mathbf{95.79}$ & $97.47$ & $\mathbf{99.44}$ & $89.52$ & & $97.22$ & $97.39$ & & $97.29$ \\
        Llama 3 & $8$B & $\mathbf{97.91}$ & $\mathbf{98.54}$ & & $\mathbf{98.56}$ & $95.36$ & $\mathbf{98.58}$ & $99.33$ & $\mathbf{91.43}$ & & $\mathbf{98.57}$ & $\mathbf{97.42}$ & & $\mathbf{98.07}$ \\
        \bottomrule
    \end{tabular}
    \caption{Experimental results of our proposed models trained with TabMWP and TabMWP-TeLL against baselines. * denotes the estimated size of GPT-4 \cite{bambhaniya2024demystifying}.}
    \label{tab:results}
\end{table*}

==> Tables/Statistics.tex <==
\begin{table}[t!]
    \centering
    \small
    \begin{tabular}{l|cccc}
        \toprule
         & \textbf{Train} & \textbf{Valid} & \textbf{Test} & \textbf{Total} \\
         \midrule
        \#Question & $23,059$ & $7,686$ & $7,686$ & $38,431$ \\
        \#Free-text & $17,135$ & $5,710$ & $5,694$ & $28,719$ \\
        \#MCQ & $5,744$ & $1,976$ & $1,992$ & $9,712$ \\
        \midrule
        \#Table & $22,620$ & $7,546$ & $7,549$ & $37,644$ \\
        \#Solution & $21,623$ & $7,365$ & $7,378$ & $35,442$ \\
        \bottomrule
    \end{tabular}
    \caption{Statistics of the TabMWP dataset.}
    \label{tab:statistics}
\end{table}

==> Tables/Step-by-Step.tex <==
\begin{table}[t!]
    \centering
    \begin{tabular}{l|ccc}
        \toprule
        \textbf{Data} & \textbf{Qwen} & \textbf{Llama 3} & \textbf{Mistral} \\
        \midrule
        TabMWP & $93.59$ & $94.29$ & $90.00$ \\
        TabMWP + XXX & $95.55$ & $95.54$ & $90.00$ \\
        XXX & $95.86$ & $96.21$ & $90.00$ \\
        \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:sbs}
\end{table}
